Phase Retrieval from Local Measurements: Improved Robustness via Eigenvector-Based Angular Synchronization

We improve a phase retrieval approach that uses correlation-based measurements with compactly supported measurement masks [27]. The improved algorithm admits deterministic measurement constructions together with a robust, fast recovery algorithm that consists of solving a system of linear equations in a lifted space, followed by finding an eigenvector (e.g., via an inverse power iteration). Theoretical reconstruction error guarantees from [27] are improved as a result for the new and more robust reconstruction approach proposed herein. Numerical experiments demonstrate robustness and computational efficiency that outperforms competing approaches on large problems. Finally, we show that this approach also trivially extends to phase retrieval problems based on windowed Fourier measurements.

==> Perturb_V2.tex <==
\BPnote{The result at the end of this section is a $C \dfrac{\eta d^3}{\delta^{5/2}}$, whereas the graph method gives us $C' \dfrac{\eta d^{5/2}}{\delta^2}$.  I really can't imagine a situation where we'd want the extra $(d / \delta)^{1/2}$ at the moment...  Should we trim this section?}

In this section we develop the perturbation results necessary in order to understand the performance of line 5 of Algorithm~\ref{alg:phaseRetrieval}.
%\subsection{General Perturbation Results}
We will begin with a general perturbation result concerning the top eigenvector of a generic Hermitian matrix.  %Note that the bound we obtain depends only on the spectral gap of the unperturbed matrix $\X_0$, as opposed to the type of bound obtained via a straightforward application of, e.g., the $\sin \theta$ theorem \cite{davis1970rotation,stewart1990matrix}.

\begin{lem}
Let $\X_0 = \sum^d_{j=1} \nu_j \x_j\x_j^*$ be Hermitian with eigenvalues $\nu_1 \geq \nu_2 \geq \dots \geq \nu_d$ and orthonormal eigenvectors $\x_1, \dots, \x_d \in \mathbbm{C}^d$.  Suppose that $\X = \sum^d_{j=1} \lambda_j \v_j\v_j^*$ is Hermitian with eigenvalues $\lambda_1 \geq \lambda_2 \geq \dots \geq \lambda_d$, orthonormal eigenvectors $\v_1, \dots, \v_d \in \mathbbm{C}^d$, and $\Vert \X-\X_0 \Vert_{\rm F}~\leq \eta \Vert \X_0 \Vert_F$ for some $\eta \geq 0$.  Then, %there exists a $\theta \in [0, 2 \pi]$ such that
\[ \left( 1 - | \langle \x_1, \v_1 \rangle |^2 \right)  \leq  \frac{4 \eta^2 \Vert \X_0 \Vert^2_{\rm F} }{(\nu_1- \nu_2)^2} .\]
%whenever $2\eta \Vert \X_0 \Vert_F \leq |\nu_1 - \nu_2|$.  
%%If $\lambda_2 = \nu_2$ always holds (as per \S\ref{sec:Spectrum} with $\X_0 = \tilde{\X}_0$ and $\X = \tilde{\X}$) then \[ \left( 1 - | \langle \x_1, \v_1 \rangle |^2 \right)  \leq  \frac{\eta^2 \Vert \X_0 \Vert^2_{\rm F} }{(\nu_1- \nu_2)^2}. \]
%%will hold for all $\eta \geq 0$.
        \label{lem:GenBound}
\end{lem}

\begin{proof}
An application of the $\sin \theta$ theorem \cite{davis1970rotation,stewart1990matrix} (see, e.g., the proof of Corollary 1 in \cite{yu2015useful}) tells us that 
\begin{equation*}
\sin \left( \arccos \left( | \langle \x_1, \v_1 \rangle | \right) \right) \leq \frac{2 \eta \Vert \X_0 \Vert_F}{|\nu_1 - \nu_2|}.
\label{equ:SinthetaApp}
\end{equation*}
Squaring both sides we then learn that 
\begin{equation}
 \left( 1 - | \langle \x_1, \v_1 \rangle |^2 \right)  = \sin^2 \left( \arccos \left( | \langle \x_1, \v_1 \rangle | \right) \right) \leq \frac{4 \eta^2 \Vert \X_0 \Vert^2_F}{(\nu_1 - \nu_2)^2},
\label{equ:SinthetaApp}
\end{equation}
%%Considering the denominator, we can see that 
%%$$|\nu_1 - \lambda_2| \geq |\nu_1 - \nu_2| - |\nu_2 - \lambda_2| \geq |\nu_1 - \nu_2| -  \eta \Vert \X_0 \Vert_F$$
%%by Weyl's inequality (see, e.g., \cite{horn2012matrix}).  Thus, $|\nu_1 - \lambda_2| \geq \frac{|\nu_1 - \nu_2|}{2}$ whenever $2\eta \Vert \X_0 \Vert_F \leq |\nu_1 - \nu_2|$
giving us the desired inequality.  
%%For the second inequality we simply use $\lambda_2 = \nu_2$ in \eqref{equ:SinthetaApp}.
\end{proof}

The following variant of Lemma~\ref{lem:GenBound} concerning rank 1 matrices $\X_0$ is of use in the analysis of many other phase retrieval methods, and can be used, e.g., to correct and simplify the proof of equation (1.8) in Theorem 1.3 of \cite{candes2014solving}.

\begin{lem}
Let $\x_0 \in \mathbb C^d$, set $\X_0 = \x_0\x_0^*$, and let 
$\X \in \mathbb C^{d \times d}$ be Hermitian with $\Vert \X~-~\X_0 \Vert_F~\leq \eta
\Vert \X_0 \Vert_F = \eta \Vert \x_0\Vert_2^2$ for some $\eta \geq 0$.  Furthermore, let $\lambda_i$ be the $i$-th largest magnitude
eigenvalue of $\X$ and $\v_i \in \mathbb{C}^d$ an associated eigenvector, such 
that the $\v_i$ form an orthonormal eigenbasis. Then
\[ \min_{\theta \in [0, 2 \pi]} \Vert  \mathbbm{e}^{\mathbbm{i} \theta}  \x_0 - \sqrt{ 
    |\lambda_1 |} \v_1 \Vert_2 \leq (1+2 \sqrt{2}) \eta \Vert \x_0 
        \Vert_2.\footnote{It is interesting to note that similar bounds can also be obtained using simpler techniques (see, e.g., \cite{CandesFix}).} \]
        \label{cor:rank1Bound}
\end{lem}

\begin{proof}
In this special case of Lemma~\ref{lem:GenBound} we have $\nu_1 = \Vert \X_0 \Vert_F = \Vert \x_0\Vert_2^2$ and $\x_1 := \x_0 / \Vert \x_0 \Vert$.  Choose $\phi \in [0, 2 \pi]$ such that $\langle \mathbbm{e}^{\mathbbm{i} \phi} \x_0, \v_1 \rangle  = \vert \langle  \x_0, \v_1 \rangle \vert$.  Then, 
%
\begin{align}
 \Vert \mathbbm{e}^{\mathbbm{i} \phi} \x_0 - \sqrt{\nu_1} \v_1 \Vert_2^2 &= 2\nu_1 - 2 \nu_1  \cdot \vert \langle  \x_0 / \Vert \x_0 \Vert, \v_1 \rangle \vert = 2\nu_1 - 2 \nu_1  \cdot \vert \langle  \x_1, \v_1 \rangle \vert \nonumber \\ &\leq 2 \nu_1 \left( 1 - \vert \langle  \x_1, \v_1 \rangle \vert \right) \left( 1 + \vert \langle  \x_1, \v_1 \rangle \vert \right) \label{equ:CorIntermed} \\ &= 2 \nu_1 \left( 1 - | \langle \x_1, \v_1 \rangle |^2 \right) \leq 8 \eta^2 \Vert \X_0 \Vert_{\rm F} \nonumber
\end{align}
where the last inequality follows from Lemma~\ref{lem:GenBound} with $\nu_1 = \Vert \X_0 \Vert_F = \Vert \x_0\Vert_2^2$.  Finally, by the triangle inequality, Weyl's inequality (see, e.g., \cite{horn2012matrix}), and \eqref{equ:CorIntermed}, we have
\begin{align*}
  \Vert \mathbbm{e}^{\mathbbm{i} \phi} \x_0 - \sqrt{ |\lambda_1|} \v_1 \Vert_2 & \leq \Vert 
    \mathbbm{e}^{\mathbbm{i} \phi} \x_0 -\sqrt \nu_1 \v_1 \Vert_2 + \Vert \sqrt \nu_1 \v_1 - 
    \sqrt{|\lambda_1|} \v_1 \Vert_2 \\
    & \leq 2 \sqrt{2} \cdot \eta \sqrt \nu_1 + \left \vert \sqrt \nu_1 - \sqrt{|\lambda_1|} \right \vert \\ & \leq 2 \sqrt{2} \cdot \eta \sqrt 
        \nu_1 + \frac{| \nu_1 - \lambda_1 |}{\sqrt \nu_1 + \sqrt{|\lambda_1|}} \\
     & \leq 2 \sqrt{2} \cdot \eta \sqrt \nu_1 + \frac{\eta \nu_1}{\sqrt \nu_1 + \sqrt{|\lambda_1|}}\\ 
    & \leq (1+2 \sqrt{2}) \eta \sqrt \nu_1.
\end{align*}
The desired result now follows.
\end{proof}

We may now use Lemma~\ref{lem:GenBound} to produce a perturbation bound for our banded matrix of phase differences $\tilde{\X}_0$ from \eqref{equ:MatrixofPhases}.

\begin{thm}
Let $\tX_0$ be the matrix of \eqref{equ:MatrixofPhases} and let $\tX$, $\tx$, and $\tx_0$  be as in Algorithm~\ref{alg:phaseRetrieval}. Suppose that $\Vert \tX_0 - \tX \Vert_F \le \eta \Vert \tX_0 \Vert_F$ 
%Let $\tilde{\X}_0$ be the Hermitian matrix from \eqref{equ:MatrixofPhases} with eigenvalues $\lambda_1 = 2 \delta - 1 \geq \ldots \ge \lambda_d$, and $\| \tilde{\X}_0 \|^2_{\rm F} = d (2 \delta - 1)$.  Let $\tilde{\X}$ be the Hermitian matrix from line 4 of Algorithm~\ref{alg:phaseRetrieval}, and suppose that $\Vert \tilde{\X} - \tilde{\X}_0 \Vert_{\rm F}~\leq \eta \Vert \tilde{\X}_0 \Vert_F$ 
for some $\eta>0$.  Then, there exists an absolute constant $C \in \mathbb{R}^+$ such that
%\[ \left( 1 - \frac{1}{d^2}| \langle \tilde{\x}_0, \tilde{\x} \rangle |^2 \right)  \leq  C \eta^2 \left( \frac{d}{\delta} \right)^5 \]
%        \label{cor2:GenBound}
%where the phase vectors $\tilde{\x}$ and $\tilde{\x}_0$ are normalized such that $\| \tilde{\x} \|_2 = \| \tilde{\x}_0 \|_2 = \sqrt{d}$.
\[\min_{\theta\in[0,2\pi]} \Vert \tx_0 - \mathbbm{e}^{\mathbbm{i}\theta} \tx \Vert_2 \le C\bigfrac{\eta d^3}{\delta^{\frac{5}{2}}}.\]

\label{cor2:GenBound}
\end{thm}

\begin{proof}
Recall that the phase vectors $\tilde{\x}$ and $\tilde{\x}_0$ are entrywise normalized so that $\| \tilde{\x} \|_2 = \| \tilde{\x}_0 \|_2 = \sqrt{d}$.  Combining Lemmas~\ref{lem:EigGap} and \ref{lem:GenBound} after noting that $\| \tilde{\X}_0 \|^2_{\rm F} = d (2 \delta - 1)$ we learn that 
\begin{equation}
\left( 1 - \frac{1}{d^2}| \langle \tilde{\x}_0, \tilde{\x} \rangle |^2 \right)  \leq  C' \eta^2 \left( \frac{d}{\delta} \right)^5
\label{equ:cor2GenBIP}
\end{equation}
for an absolute constant $C' \in \mathbb{R}^+$.  Let $\phi \in [0,2 \pi)$ be such that $\Re\left( \langle \tilde{\x}_0,\mathbbm{e}^{\mathbbm{i} \phi} \tilde{\x} \rangle \right) = \left| \langle \tilde{\x}_0, \tilde{\x} \rangle \right|$.  Then,
\begin{align*}
\| \tilde{\x}_0 - \mathbbm{e}^{\mathbbm{i} \phi} \tilde{\x} \|^2_2 &= 2d - 2 \Re\left( \langle \tilde{\x}_0,\mathbbm{e}^{\mathbbm{i} \phi} \tilde{\x} \rangle \right) \\
&= 2d \left( 1 - \frac{1}{d} \left| \langle \tilde{\x}_0, \tilde{\x} \rangle \right| \right) \leq 2d \left( 1 - \frac{1}{d^2} \left| \langle \tilde{\x}_0, \tilde{\x} \rangle \right|^2 \right).
\end{align*}
Combining this last inequality with \eqref{equ:cor2GenBIP} concludes the proof.
\end{proof}

%%%\begin{lem}
%%%Let $\X_0 = \sum^d_{j=1} \nu_j \x_j\x_j^*$ be Hermitian with eigenvalues $\nu_1 \geq |\nu_2| \geq \dots \geq |\nu_d|$, $\nu_1 > 0$, and orthonormal eigenvectors $\x_1, \dots, \x_d \in \mathbbm{C}^d$.  Suppose that $\X = \sum^d_{j=1} \lambda_j \v_j\v_j^*$ is Hermitian with eigenvalues $|\lambda_1| \geq |\lambda_2| \geq \dots \geq |\lambda_d|$, orthonormal eigenvectors $\v_1, \dots, \v_d \in \mathbbm{C}^d$, and $\Vert \X-\X_0 \Vert_{\rm F}~\leq \eta \Vert \X_0 \Vert_F$ for some $\eta>0$.  Then, %there exists a $\theta \in [0, 2 \pi]$ such that
%%%\[ \left( 1 - | \langle \x_1, \v_1 \rangle |^2 \right)  \leq  \frac{3 \eta(\frac{3}{2} \eta +1 )\Vert \X_0 \Vert^2_{\rm F} }{\nu_1(\nu_1- |\nu_2|)} \]
%%%        \label{lem:GenBound}
%%%\end{lem}
%%%
%%%%Note that a straightforward application of the $\sin \theta$ theorem based on an arbitrary perturbation in the Frobenius norm as per Lemma~\ref{lem:GenBound} gives the bound 
%%%%$$\left( 1 - | \langle \x_1, \v_1 \rangle |^2 \right)  \leq \frac{\eta^2 \Vert \X_0 \Vert^2_{\rm F}}{(\nu_1- |\nu_2|)^2}.$$
%%%%Comparing this to the conclusion of Lemma~\ref{lem:GenBound}, we can see that Lemma~\ref{lem:GenBound} provides a better upper bound whenever $\eta > \frac{6(\nu_1- |\nu_2|)}{2\nu_1 - 9(\nu_1- |\nu_2|)}$.  
%%%
%%%\begin{proof}
%%%Consider that 
%%%\[\begin{array}{rcl}
%%%\sqrt{\sum_{j=2}^d \lambda_j^2} - \sqrt{\sum_{j=2}^d \nu_j^2} & \le & \sqrt{\sum_{j=2}^d(\lambda_j - \nu_j)^2} \\
%%%& \le & \sqrt{\sum_{j=1}^d(\lambda_j - \nu_j)^2} \\
%%%& \le & \eta||X_0||_{\rm F}, 
%%%\end{array}.\]
%%%where the first inequality comes from the triangle inequality and the last comes from the Wielandt-Hoffman inequality \cite{hoffman1953variation}.  This gives
%%%\[ \sqrt{\sum_{j=2}^d \lambda_j^2} \le \sqrt{\sum_{j=2}^d \nu_j^2} + \eta ||X_0||_{\rm F}.\]
%%%
%%%% Let $V \in \mathbbm{C}^{d \times d}$ be the unitary matrix with $v_j$ as its $j^{\rm th}$ column, and let $\Lambda \in \mathbbm{R}^{d \times d}$ be a diagonal matrix whose $j^{\rm th}$ diagonal entry is $\lambda_j$.  We have that
%%%% \begin{align*}
%%%%  \sqrt{\sum^d_{j=2} \lambda^2_j }&\leq \sqrt{2 \lambda^2_1 + \sum^d_{j = 2} \lambda^2_j - 2 \lambda_1 \sum^d_{j=1} \lambda_j \left| \left(  V^* \x_1 \right)_j \right|^2} \\ 
%%%%  &= \sqrt{\Vert \X \Vert^2_{\rm F} - 2 \lambda_1{\rm Trace} \left(\Lambda (V^* x_1)(V^* x_1)^* \right) + \lambda^2_1}\\ 
%%%%  &= \Vert \Lambda - \lambda_1 (V^* \x_1)(V^* \x_1)^* \Vert_{\rm F} \\
%%%%  &= \Vert \X - \lambda_1 \x_1 \x^*_1 \Vert_{\rm F} \\
%%%%  & \leq \Vert \X - \X_0 \Vert_{\rm F} +  \Vert \X_0 - \nu_1  \x_1 \x^*_1 \Vert_{\rm F} +  \Vert \nu_1  \x_1 \x^*_1 - \lambda_1 \x_1 \x^*_1 \Vert_{\rm F}\\
%%%%  &\leq 2 \eta \Vert \X_0 \Vert_{\rm F} + \sqrt{\sum^d_{j=2} \nu^2_j },
%%%%  \end{align*}
%%%% where the last inequality uses our assumption, and Weyl's inequality.  
%%%As a result, we have that
%%%\begin{align*}
%%% \Vert \X_0 - \nu_1 \v_1 \v^*_1 \Vert_{\rm F} &\leq  \Vert \X_0 - \X \Vert_{\rm F} + \Vert \X- \nu_1 \v_1 \v^*_1 \Vert_{\rm F} \\
%%% & \leq \eta \Vert \X_0 \Vert_{\rm F} + \left \Vert (\lambda_1- \nu_1 ) \v_1 \v^*_1 + \sum^d_{j=2} \lambda_j \v_j\v_j^* \right \Vert_{\rm F}\\
%%% & \leq 2 \eta \Vert \X_0 \Vert_{\rm F} +  \sqrt{\sum^d_{j=2} \lambda^2_j }
%%% \end{align*}
%%%using our assumption and Weyl's inequality (see, e.g., \cite{horn2012matrix}).  Finally, we may now use our previous bound to obtain
%%%\begin{equation}
%%%\Vert \X_0 - \nu_1 \v_1 \v^*_1 \Vert_{\rm F}  \leq 3 \eta \Vert \X_0 \Vert_{\rm F} + \sqrt{\sum^d_{j=2} \nu^2_j }.
%%%\label{equ:FrobBB}
%%%\end{equation}
%%%
%%%Expanding this last norm we obtain
%%%\begin{align*}
%%% \Vert \X_0 - \nu_1 \v_1 \v^*_1 \Vert^2_{\rm F} &=  \Vert \X_0 \Vert^2_{\rm F} - 2 \nu_1 {\rm Trace} \left(  \X^*_0 \v_1 \v^*_1\right) + \nu^2_1\\
%%% &= \sum^d_{j=1} \nu^2_j - 2 \nu_1 \sum_{j=1}^d \nu_j | \langle \x_j, \v_1 \rangle |^2 + \nu^2_1\\
%%% &= 2 \nu^2_1 \left( 1 - | \langle \x_1, \v_1 \rangle |^2 \right) + \sum^d_{j=2} \nu^2_j - 2 \nu_1 \sum_{j=2}^d \nu_j | \langle \x_j, \v_1 \rangle |^2.
%%%\end{align*}
%%%Thus, we have that
%%%\begin{align*}
%%%2 \nu^2_1 \left( 1 - | \langle \x_1, \v_1 \rangle |^2 \right) &=  \Vert \X_0 - \nu_1 \v_1 \v^*_1 \Vert^2_{\rm F} + 2 \nu_1 \sum_{j=2}^d \nu_j | \langle \x_j, \v_1 \rangle |^2 - \sum^d_{j=2} \nu^2_j \\
%%%&\leq \Vert \X_0 - \nu_1 \v_1 \v^*_1 \Vert^2_{\rm F} + 2 \nu_1 |\nu_2| \sum_{j=2}^d | \langle \x_j, \v_1 \rangle |^2 - \sum^d_{j=2} \nu^2_j \\
%%%&= \Vert \X_0 - \nu_1 \v_1 \v^*_1 \Vert^2_{\rm F} + 2 \nu_1 |\nu_2| \left( 1 - | \langle \x_1, \v_1 \rangle |^2 \right) - \sum^d_{j=2} \nu^2_j.
%%%\end{align*}
%%%Rearranging once more, we have that
%%%$$(2 \nu^2_1- 2 \nu_1 |\nu_2| ) \left( 1 - | \langle \x_1, \v_1 \rangle |^2 \right) \leq \Vert \X_0 - \nu_1 \v_1 \v^*_1 \Vert^2_{\rm F} - \sum^d_{j=2} \nu^2_j.$$
%%%Using $\eqref{equ:FrobBB}$ now gives us that
%%%\begin{align}
%%%\left( 1 - | \langle \x_1, \v_1 \rangle |^2 \right) &\leq \frac{\left( 3 \eta \Vert \X_0 \Vert_{\rm F} + \sqrt{\sum^d_{j=2} \nu^2_j }\right)^2  - \sum^d_{j=2} \nu^2_j}{2 \nu^2_1- 2 \nu_1 |\nu_2|} \nonumber \\
%%%&= \frac{9 \eta^2 \Vert \X_0 \Vert^2_{\rm F} + 6 \eta \Vert \X_0 \Vert_{\rm F} \left( \sqrt{ \Vert \X_0 \Vert^2_{\rm F} - \nu^2_1 } \right) }{2 \nu^2_1- 2 \nu_1 |\nu_2|} \label{equ:DetailedGenBound}\\
%%%&\leq \frac{3 \eta(\frac{3}{2} \eta +1 )\Vert \X_0 \Vert^2_{\rm F} }{\nu_1(\nu_1- |\nu_2|)}. \nonumber
%%%\end{align}
%%%The stated result follows.
%%%\end{proof}
%%%
%%%The following varaint of Lemma~\ref{lem:GenBound} concerning rank 1 matrices $\X_0$ is of use in the analysis of many other phase retrieval methods, and can be used, e.g., to correct and simplify the proof of equation (1.8) in Theorem 1.3 of \cite{candes2014solving}.
%%%
%%%\begin{lem}
%%%Let $\x_0 \in \mathbb C^d$, set $\X_0 = \x_0\x_0^*$, and let 
%%%$\X \in \mathbb C^{d \times d}$ be Hermitian with $\Vert \X~-~\X_0 \Vert_F~\leq \eta
%%%\Vert \X_0 \Vert_F = \eta \Vert \x_0\Vert_2^2$ for some 
%%%$\eta>0$.  Furthermore, let $\lambda_i$ be the $i$-th largest magnitude
%%%eigenvalue of $\X$ and $\v_i \in \mathbb{C}^d$ an associated eigenvector, such 
%%%that the $\v_i$ form an orthonormal eigenbasis. Then
%%%\[ \min_{\theta \in [0, 2 \pi]} \Vert  \mathbbm{e}^{\mathbbm{i} \theta}  \x_0 - \sqrt{ 
%%%    |\lambda_1 |} \v_1 \Vert_2 \leq 4 \eta \Vert \x_0 
%%%        \Vert_2.\footnote{The constant 4 here is certainly not optimal, and can be improved slightly by using different arguments (see, e.g., \cite{CandesFix}).} \]
%%%        \label{cor:rank1Bound}
%%%\end{lem}
%%%
%%%\begin{proof}
%%%In this special case of Lemma~\ref{lem:GenBound} we have $\nu_1 = \Vert \X_0 \Vert_F = \Vert \x_0\Vert_2^2$ and $\x_1 = \x_0 / \Vert \x_0 \Vert$.  Choose $\phi \in [0, 2 \pi]$ such that $\langle \mathbbm{e}^{\mathbbm{i} \phi} \x_0, \v_1 \rangle  = \vert \langle  \x_0, \v_1 \rangle \vert$.  Then, 
%%%%
%%%\begin{align}
%%% \Vert \mathbbm{e}^{\mathbbm{i} \phi} \x_0 - \sqrt{\nu_1} \v_1 \Vert_2^2 &= 2\nu_1 - 2 \nu_1  \cdot \vert \langle  \x_0 / \Vert \x_0 \Vert, \v_1 \rangle \vert = 2\nu_1 - 2 \nu_1  \cdot \vert \langle  \x_1, \v_1 \rangle \vert \nonumber \\ &\leq 2 \nu_1 \left( 1 - \vert \langle  \x_1, \v_1 \rangle \vert \right) \left( 1 + \vert \langle  \x_1, \v_1 \rangle \vert \right) \label{equ:CorIntermed} \\ &= 2 \nu_1 \left( 1 - | \langle \x_1, \v_1 \rangle |^2 \right) \leq 9 \eta^2 \Vert \X_0 \Vert_{\rm F} \nonumber
%%%\end{align}
%%%where the last inequality follows from \eqref{equ:DetailedGenBound} with $\nu_1 = \Vert \X_0 \Vert_F = \Vert \x_0\Vert_2^2$.  Finally, by the triangle inequality, Weyl's inequality, and \eqref{equ:CorIntermed}, we have
%%%\begin{align*}
%%%  \Vert \mathbbm{e}^{\mathbbm{i} \phi} \x_0 - \sqrt{ |\lambda_1|} \v_1 \Vert_2 & \leq \Vert 
%%%    \mathbbm{e}^{\mathbbm{i} \phi} \x_0 -\sqrt \nu_1 \v_1 \Vert_2 + \Vert \sqrt \nu_1 \v_1 - 
%%%    \sqrt{|\lambda_1|} \v_1 \Vert_2 \\
%%%    & \leq 3 \eta \sqrt \nu_1 + \left \vert \sqrt \nu_1 - \sqrt{|\lambda_1|} \right \vert \\ & \leq 3 \eta \sqrt 
%%%        \nu_1 + \frac{| \nu_1 - \lambda_1 |}{\sqrt \nu_1 + \sqrt{|\lambda_1|}} \\
%%%     & \leq 3 \eta \sqrt \nu_1 + \frac{\eta \nu_1}{\sqrt \nu_1 + \sqrt{|\lambda_1|}}\\ 
%%%    & \leq 4 \eta \sqrt \nu_1.
%%%\end{align*}
%%%The desired result now follows.
%%%\end{proof}
%%%
%%%We may now use Lemma~\ref{lem:GenBound} to produce a perturbation bound for our banded matrix of phase differences $\tilde{\X}_0$ from \eqref{equ:MatrixofPhases}.
%%%
%%%\begin{thm}
%%%Let $\tilde{\X}_0$ be the Hermitian matrix from \eqref{equ:MatrixofPhases} with eigenvalues $\lambda_1 = 2 \delta - 1 \geq \dots$, and $\| \tilde{\X}_0 \|^2_{\rm F} = d (2 \delta - 1)$.  Let $\tilde{\X}$ be the Hermitian matrix from line 4 of Algorithm~\ref{alg:phaseRetrieval}, and suppose that $\Vert \tilde{\X} - \tilde{\X}_0 \Vert_{\rm F}~\leq \eta \Vert \tilde{\X}_0 \Vert_F$ for some $\eta>0$.  Then, there exists an absolute constant $C \in \mathbb{R}^+$ such that
%%%\[ \left( 1 - \frac{1}{d^2}| \langle \tilde{\x}_0, \tilde{\x} \rangle |^2 \right)  \leq  C \left( \eta^2 + \frac{2}{3} \eta \right) \left( \frac{d}{\delta} \right)^3 \]
%%%        \label{cor2:GenBound}
%%%where the phase vectors $\tilde{\x}$ and $\tilde{\x}_0$ are normalized such that $\| \tilde{\x} \|_2 = \| \tilde{\x}_0 \|_2 = \sqrt{d}$.
%%%\label{cor2:GenBound}
%%%\end{thm}
%%%
%%%\begin{proof}
%%%Combine Lemmas~\ref{lem:EigGap} and \ref{lem:GenBound}.
%%%\end{proof}
%% kron stuff %%

